Sound-Word2Vec: Learning Word Representations Grounded in Sounds

To be able to interact better with humans, it is crucial for machines to understand sound - a primary modality of human perception. Previous works have used sound to learn embeddings for improved generic textual similarity assessment. In this work, we treat sound as a first-class citizen, studying downstream textual tasks which require aural grounding. To this end, we propose sound-word2vec - a new embedding scheme that learns specialized word embeddings grounded in sounds. For example, we learn that two seemingly (semantically) unrelated concepts, like leaves and paper are similar due to the similar rustling sounds they make. Our embeddings prove useful in textual tasks requiring aural reasoning like text-based sound retrieval and discovering foley sound effects (used in movies). Moreover, our embedding space captures interesting dependencies between words and onomatopoeia and outperforms prior work on aurally-relevant word relatedness datasets such as AMEN and ASLex.

==> sections/approach_outline.tex <==
Input/Output
\begin{itemize}
	\item Input to the model (at training) is a set of tags (words) $\mathbb{T}$ and a sound $v$ associated with them.
	\item Our model learns embeddings for words $t_i$ that are grounded in the sounds. 
	\item The output of our model is the set of trained embeddings for words.
\end{itemize}
Clustering
\begin{itemize}
\item The key idea in sound-word2vec is to have words which sound similar closer in the embedding space.
\item To do this, we first need to discover sounds which are similar to each other.
\item We discover similar concepts in sound by clustering the sounds, this is similar to previous work on using surrogate supervision for multimodal tasks.
\item We use the clustered sounds as supervision for training word embeddings. In practice, we do the clustering using K-means with $K$ set as a hyperparameter.
\end{itemize}
Sound Word2Vec Model
\begin{itemize}
	\item Let the vocabulary size be $N$, cluster size be $K$.
	\item Let $G(v)$ be the inferred cluster-id for a sound $v$.
	\item Let $W_p \in \mathbb{R}^{N\times D}$ be the embedding or projection matrix, which projects a word to a $D$ dimensional embedding.
	\item Given a training instance $\{T, v\}$, we encode each of the words using the vocabulary $N$, by placing a 1 at the entry corresponding to the word.
	\item We then project each of the words into the embedding to get a set of vectors $\{W_{p}^{t}\}$. The overall representation for the set of words is the average of the vectors: $W_{p}^{T} = \sum_{t \in T} W_{p}^{t}$.
	\item Given this representation for the set of tags, we multiply it by an output weight matrix $W_{o} \in \mathbb{R}^{D \times K}$. Following this, we apply the softmax function to form a distribution. We train to maximize the likelihood of the correct (surrogate class) for the sound conditioned on the textual input. That is, $\max_{W_p, W_o} \log P(G(v) | T; W_{p}, W_{o})$.
	\item The output of the training procedure is the projection matrix $W_p$.
\end{itemize}
Initialization
\begin{itemize}
	\item We initialize the projection matrix with word2vec embeddings~\cite{add}.
	\item This allows us induce smoothness in the sound embeddings. We can reason about the sounds of words which we might not have seen explicitly with sounds in training.
	\item It also allows us to use a larger vocabulary (~3M) while fine-tuning for words which have associated sounds.
\end{itemize}
Feature Space for Clustering
\begin{itemize}
	\item blah
\end{itemize}
Intuitions for the model \rama{can add the stuff on the board}
Relations to Word2Vec
\begin{itemize}
	\item The sound-word2vec model has close relation to the Continuous Bag of Words (CBOW)~\cite{add} word2vec model.
	\item In the CBOW model, given a set of n-grams in context (as opposed to a bag of tags), a held out word (which appears in context) is supplied as surrogate supervision, as opposed to the surrogate sound class index.
	\item Thus, embeddings for words which appear in similar contexts become similar.
\end{itemize}


==> sections/discussion_outline.tex <==
\begin{itemize}
	\item In this work we proposed a novel sound-word2vec embedding which bridges the semantic gap between sound and language.
	\item Our embeddings capture rich notions of similarity grounded in language.
	\item We show that our embeddings capture semantics as well as sound similarity by showing better results on the text-based sound retireval task.
	\item We find that our embeddings are able to recover folly sounds used for special effects in movies.
	\item We find that our embeddings are not only able to reason about similarities between objects/words that sound similar, but also give insights into onamotopia words for various concepts/objects.
	\item In contrast to onamotopia (as a representation of sound), our continuous valued word embeddings can capture richer noitions of semantic similarity.
\end{itemize}



==> sections/intro_outline.tex <==
P1
\begin{itemize}
\item Sound/acoustics and Vision are of our primary modes of interaction with the world.
\item We describe our experiences / communicate ideas through language.
\item A lot of language seems to have evolved to describe ideas/characteristics of our physical world.
\item There is a rich suite of words that we have specialized to describe visual properties of objects.
\item We might describe the cat in the image as (furry, green-eyed, etc.)
\item Thus, given the visual instantiation of the cat, we have a lot of ways to communicate about it, in terms of shared, attribute-like properties.
\item Take for example, the image in Fig. 1 (compare mental image to fig.1.)
\end{itemize}

P2
\begin{itemize}
\item But, how would we describe the auditory instantiation of a cat?
\item One notion is to describe it in terms of the waveform/signal of the sound
\item But that is not high-level, it is not intuitive for everyday usage.
\item To bridge this gap, we have come up with words like ``meow'', which describe/phonetically mimic the particular sound made by a cat -onaemoptopia.
\item However, we still find it hard to communicate about many sounds that might not be frequent/ worth talking about.
\item In some cases, especially depending on the language, it might even be hard to phrase some sounds as words (\rama{add examples})
\item For instance, how do we describe the sound of a celery stick breaking (is it crack, snap, or crunch)?
\end{itemize}

P3
\begin{itemize}
\item In this work, we want to bridge this gap (\rama{some name for this phenomena, beyond gap?}) between sound and language.
\item Recent work has focussed on language understanding through embeddings - explain embeddings.
\item More specifically, we learn embeddings for words that are grounded in the sounds associated with them (without the need for an intermediate onaemotopia representation.)
\item That is, if two words are associated with similar sounds, their embeddings should also be similar.
\item Thus, we might realize in the embedding that the sound of a celery stick breaking as similar to a carrot breaking, for instance.
\item This is something that we as humans also do.
\end{itemize}

P4
\begin{itemize}
\item We learn representations for words grounded in sound.
\item We show that the embeddings we learn help retrieve sound from descriptions better than baseline word2vec representations in a text-based sound retrieval task.
\item We use our embeddings to discover or suggest pholly (\rama{is this the right spelling?}) sounds (such as those used for special effects in movies). For instance, we recover that the effect of breaking bones can be created from celery sticks (\ashwin{check if this is true}).
\end{itemize}


==> sections/related_outline.tex <==
We next discuss related work in learning word embeddings, multi-modal learning with surrogate supervision, and onomatopoeia.

Onomatopoeia
\begin{itemize}
	\item Traditional tool in language to bridge the gap to sound
	\item Theories of language bow-wow even suggest that onamotopeoia is how language got created
	\item Consequently, it has received a lot of attention
	\item Vector based representation of onamotopoeia words paper
	\item On top of this, we have a richer continuous representation that directly reasons about similarity in sound, as opposed to an intermediate language representation like ontopia -- as a result we can analyze much larger set of words.
	\item We are different in that we are not limited by onamotopoeia, we learn distributed representations for words.
	\item Indeed, we can embed on-topia words and regular words into the vector space to discover ontopia for words.
\end{itemize}

Word Embeddings
\begin{itemize}
	\item neural network language model, idea is to predict the likelihood of a word in the context of other words
	\item word2vec, glove, etc.
	\item in contrast to these we are interested in learning embeddings for words grounded in sound.
	\item audio word2vec analyszes phonemes, while we are interested in the actual sounds produced by the objects.
	\item Give example of how why we are different.
\end{itemize}


Multimodal learning through surrogate supervision.
\begin{itemize}
	\item Visual Word2Vec
	\item Andrew Owens ECCV paper
	\item In contrast to visual word2vec, we want to learn embeddings for words, grounded in sound, while ECCV paper wants to learn embeddings for images grounded into sound.
	\item Learning sound grounded text embeddings helps us perform tasks like text-based sound retrieval, discovering foley sounds etc.
\end{itemize}


==> sections/results_outline.tex <==
Baselines
\begin{itemize}
\item word2vec trained on Google News Dataset~\cite{}
\item word2vec trained on collections of tags from the Freesound database~\cite{}
\item sound-word2vec-random: randomly initialized sound-word2vec
\item sound-word2vec: soundword2vec intitialized from word2vec
\item we use word-embeddings to refer to all of the above below.
\end{itemize}

Tasks
A filler sentence about the tasks.

Text-based sound retrieval
\begin{itemize}
\item We provide quantitative results on text-based sound retrieval task.
\item Given a description of a sound in a sentence, the task is to retrieve the sound corresponding to the sentence.
\item In a sense, this task captures exactly what we want to accomplish: briding the gap between language and sound.
\item We use the tags associated with sounds in the Freesound dataset to perform the retrieval.
\item In practice, we average the sound-word2vec embeddings for all the words in the sentence (in the vocabulary), and the sound-word2vec embeddings for all the tags, and compute the consine similarity to score a sound.
\item We rank sounds based on the score.
\item We use all the baselines from the previous paragraph, and evaluate them using retrieval metrics (Recall@1, Recall@10, Recall@50, Recall@100, medR)
\item We find that sound-word2vec does better than baselines (Table.1)
\end{itemize}

% \begin{table}[h!]
% \centering
% \begin{tabular}{c  c c c c}\toprule
% \textbf{Embedding} & \textbf{recall@1} & \textbf{recall@10} & \textbf{recall&50} & \textbf{recall&100} \\
% \midrule
% w2v & 6.47 & 14.25 & 17.41 & 26.03 \\
% tag-w2v & 6.95 & 15.10 & 18.53  & 27.21  \\
% sound-w2v & 6.49 & 14.98 & 18.01 & 26.43 \\
% (no pretraining) &   &   &   &   \\
% sound-w2v & \textbf{7.11} & \textbf{15.88} & \textbf{19.34} & \textbf{28.67} \\
% \bottomrule
% \end{tabular}
% \caption{Quantitative results for the sound retrieval task with user-provided sentence descriptions as query.}
% \label{tab:retrieval}
% \end{table} 

\begin{table}\tiny
    \centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccccc} 
    \toprule
    Embedding & \multicolumn{4}{c}{recall} \\
    \cmidrule(0.75pt){2-5}
    & @1 & @10 & @50 & @100 \\
    \midrule
    w2v & 6.47 & 14.25 & 21.72 & 26.03 \\
    tag-w2v & 6.95 & 15.10 & 22.43  & 27.21  \\
    sound-w2v & 6.49 & 14.98 & 21.96 & 26.43 \\
    (no pretraining) &   &   &   &   \\
    sound-w2v & \textbf{7.11} & \textbf{15.88} & \textbf{23.14} & \textbf{28.67} \\
    \bottomrule
\end{tabular}}
\caption{Quantitative results for the sound retrieval task (in text) with user-provided sentence descriptions a query}
\label{blah}
\end{table}

Folly sounds recovery
\begin{itemize}
\item We use a curated set of 30 pairs of folly sounds. Describe in more detail.
\item We compare the two best approaches from the previous section on how well they manage to recover known folly sound pairs
\item The dataset contains a target sound, and a sentence description of a procedure to mimic that sound.
\item From the sentence description, we compute the representation by averaging the word embeddings, and check the similarity between the target sound and the representation.
\item We repeat this procedure for all pairs of sound-tags in the validation set.
\item We check the percentile of the folly sound among the set of all pairwise similarities.
\item A better method should have a higher rank.
\end{itemize}

Qualitative Results
\begin{itemize}
\item We show some qualitative results on folly sound recovery, by showing nearest neighbors in the sound-word2vec space and the original word2vec space (Table.2)
\item We show some examples of onamotopoeia words discovered for various objects and actions in the dataset by visualizing nearest neighbours for oneamotopia words. (Fig. 2)
\end{itemize}

